Translating and evaluating single-cell Boolean network interventions in the multiscale setting

Intracellular networks process cellular-level information and control cell fate. They can be computationally modeled using Boolean networks, which are implicit-time causal models of discrete binary events. These networks can be embedded in computational agents to drive cellular behavior. To explore this integration, we construct a set of candidate interventions that induce apoptosis in a cell-survival network of a rare leukemia using exhaustive search simulation, stable motif control, and an individual-based mean field approach (IBMFA). Due to inherent algorithmic limitations, these interventions are most suitable for cell-level determinations, not the more realistic multicellular setting. To address these limitations, we treat the target control solutions as putative targets for therapeutic interventions and develop a pipeline to translate them to continuous-time multicellular, agent-based models. We set the discrete-to-continuous transitions between the Boolean network and multicellular model via thresholding and produce simple computational simulations designed to emulate situations in experimental and translational biology. These include a series of simulations: constant substrate gradients, global substrate pulses, and time-varying boundary conditions. We find that interventions that perform equally well in the implicit-time single-cell setting are separable in the multiscale setting in ability to impact population growth and spatial distribution. Further analysis shows that the population and spatial distribution differences arise from differences in internal dynamics (stable motif controls versus target controls) and network distance between the intervention and output nodes. This proof of concept work demonstrates the importance of accounting for internal dynamics in multicellular simulations as well as impacts on understanding of Boolean network control.

==> b_ycIK9GSQ <==
%apsrev4-2.bst 2019-01-14 (MD) hand-edited version of apsrev4-1.bst
%Control: key (0)
%Control: author (8) initials jnrlst
%Control: editor formatted (1) identically to author
%Control: production of article title (0) allowed
%Control: page (0) single
%Control: year (1) truncated
%Control: production of eprint (0) enabled
\begin{thebibliography}{38}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{https://doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
%</preamble>
\bibitem [{\citenamefont {Gjerga}\ \emph {et~al.}(2020)\citenamefont {Gjerga}, \citenamefont {Trairatphisan}, \citenamefont {Gabor}, \citenamefont {Koch}, \citenamefont {Chevalier}, \citenamefont {Ceccarelli}, \citenamefont {Dugourd}, \citenamefont {Mitsos},\ and\ \citenamefont {{Saez-Rodriguez}}}]{gjergaConvertingNetworksPredictive2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Gjerga}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Trairatphisan}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Gabor}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Koch}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Chevalier}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Ceccarelli}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Dugourd}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Mitsos}},\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {{Saez-Rodriguez}}},\ }\bibfield  {title} {\bibinfo {title} {Converting networks to predictive logic models from perturbation signalling data with {{CellNOpt}}},\ }\href {https://doi.org/10.1093/bioinformatics/btaa561} {\bibfield  {journal} {\bibinfo  {journal} {Bioinformatics}\ }\textbf {\bibinfo {volume} {36}},\ \bibinfo {pages} {4523} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Montagud}\ \emph {et~al.}(2022)\citenamefont {Montagud}, \citenamefont {B{\'e}al}, \citenamefont {Tobalina}, \citenamefont {Traynard}, \citenamefont {Subramanian}, \citenamefont {Szalai}, \citenamefont {Alf{\"o}ldi}, \citenamefont {Pusk{\'a}s}, \citenamefont {Valencia}, \citenamefont {Barillot}, \citenamefont {{Saez-Rodriguez}},\ and\ \citenamefont {Calzone}}]{montagudPatientspecificBooleanModels2022a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Montagud}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {B{\'e}al}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Tobalina}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Traynard}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Subramanian}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Szalai}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Alf{\"o}ldi}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Pusk{\'a}s}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Valencia}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Barillot}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {{Saez-Rodriguez}}},\ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Calzone}},\ }\bibfield  {title} {\bibinfo {title} {Patient-specific {{Boolean}} models of signalling networks guide personalised treatments},\ }\href {https://doi.org/10.7554/eLife.72626} {\bibfield  {journal} {\bibinfo
  {journal} {eLife}\ }\textbf {\bibinfo {volume} {11}},\ \bibinfo {pages} {e72626} (\bibinfo {year} {2022})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Werle}\ \emph {et~al.}(2023)\citenamefont {Werle}, \citenamefont {Ikonomi}, \citenamefont {Lausser}, \citenamefont {Kestler}, \citenamefont {Weidner}, \citenamefont {Schwab}, \citenamefont {Maier}, \citenamefont {Buchholz}, \citenamefont {Gress}, \citenamefont {Kestler},\ and\ \citenamefont {Kestler}}]{werleSystemsBiologyApproach2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~D.}\ \bibnamefont {Werle}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Ikonomi}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Lausser}}, \bibinfo {author} {\bibfnamefont {A.~M. T.~U.}\ \bibnamefont {Kestler}}, \bibinfo {author} {\bibfnamefont {F.~M.}\ \bibnamefont {Weidner}}, \bibinfo {author} {\bibfnamefont {J.~D.}\ \bibnamefont {Schwab}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Maier}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Buchholz}}, \bibinfo {author} {\bibfnamefont {T.~M.}\ \bibnamefont {Gress}}, \bibinfo {author} {\bibfnamefont {A.~M.~R.}\ \bibnamefont {Kestler}},\ and\ \bibinfo {author} {\bibfnamefont {H.~A.}\ \bibnamefont {Kestler}},\ }\bibfield  {title} {\bibinfo {title} {A systems biology approach to define mechanisms, phenotypes, and drivers in {{PanNETs}} with a personalized perspective},\ }\href {https://doi.org/10.1038/s41540-023-00283-8} {\bibfield  {journal} {\bibinfo  {journal} {npj Systems
  Biology and Applications}\ }\textbf {\bibinfo {volume} {9}},\ \bibinfo {pages} {1} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Schwab}\ \emph {et~al.}(2020)\citenamefont {Schwab}, \citenamefont {K{\"u}hlwein}, \citenamefont {Ikonomi}, \citenamefont {K{\"u}hl},\ and\ \citenamefont {Kestler}}]{schwabConceptsBooleanNetwork2020b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~D.}\ \bibnamefont {Schwab}}, \bibinfo {author} {\bibfnamefont {S.~D.}\ \bibnamefont {K{\"u}hlwein}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Ikonomi}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {K{\"u}hl}},\ and\ \bibinfo {author} {\bibfnamefont {H.~A.}\ \bibnamefont {Kestler}},\ }\bibfield  {title} {\bibinfo {title} {Concepts in {{Boolean}} network modeling: {{What}} do they all mean?},\ }\href {https://doi.org/10.1016/j.csbj.2020.03.001} {\bibfield  {journal} {\bibinfo  {journal} {Computational and Structural Biotechnology Journal}\ }\textbf {\bibinfo {volume} {18}},\ \bibinfo {pages} {571} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hemedan}\ \emph {et~al.}(2022)\citenamefont {Hemedan}, \citenamefont {Niarakis}, \citenamefont {Schneider},\ and\ \citenamefont {Ostaszewski}}]{hemedanBooleanModellingLogicbased2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~A.}\ \bibnamefont {Hemedan}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Niarakis}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Schneider}},\ and\ \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Ostaszewski}},\ }\bibfield  {title} {\bibinfo {title} {Boolean modelling as a logic-based dynamic approach in systems medicine},\ }\href {https://doi.org/10.1016/j.csbj.2022.06.035} {\bibfield  {journal} {\bibinfo  {journal} {Computational and Structural Biotechnology Journal}\ }\textbf {\bibinfo {volume} {20}},\ \bibinfo {pages} {3161} (\bibinfo {year} {2022})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rozum}\ \emph {et~al.}(2024)\citenamefont {Rozum}, \citenamefont {Campbell}, \citenamefont {Newby}, \citenamefont {Nasrollahi},\ and\ \citenamefont {Albert}}]{rozumBooleanNetworksPredictive2024}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~C.}\ \bibnamefont {Rozum}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Campbell}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Newby}}, \bibinfo {author} {\bibfnamefont {F.~S.~F.}\ \bibnamefont {Nasrollahi}},\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Albert}},\ }\bibfield  {title} {\bibinfo {title} {Boolean {{Networks}} as {{Predictive Models}} of {{Emergent Biological Behaviors}}},\ }\bibfield  {journal} {\bibinfo  {journal} {Elements in the Structure and Dynamics of Complex Networks}\ }\href {https://doi.org/10.1017/9781009292955} {10.1017/9781009292955} (\bibinfo {year} {2024})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Metzcar}\ \emph {et~al.}(2019)\citenamefont {Metzcar}, \citenamefont {Wang}, \citenamefont {Heiland},\ and\ \citenamefont {Macklin}}]{metzcarReviewCellBasedComputational2019a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Metzcar}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Wang}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Heiland}},\ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Macklin}},\ }\bibfield  {title} {\bibinfo {title} {A {{Review}} of {{Cell-Based Computational Modeling}} in {{Cancer Biology}}},\ }\href {https://doi.org/10.1200/CCI.18.00069} {\bibfield  {journal} {\bibinfo  {journal} {JCO Clinical Cancer Informatics}\ ,\ \bibinfo {pages} {1}} (\bibinfo {year} {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Chamseddine}\ and\ \citenamefont {Rejniak}(2019)}]{chamseddineHybridModelingFrameworks2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {I.~M.}\ \bibnamefont {Chamseddine}}\ and\ \bibinfo {author} {\bibfnamefont {K.~A.}\ \bibnamefont {Rejniak}},\ }\bibfield  {title} {\bibinfo {title} {Hybrid modeling frameworks of tumor development and treatment},\ }\bibfield  {journal} {\bibinfo  {journal} {Wiley Interdisciplinary Reviews: Systems Biology and Medicine}\ }\href {https://doi.org/10.1002/wsbm.1461} {10.1002/wsbm.1461} (\bibinfo {year} {2019})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Altrock}\ \emph {et~al.}(2015)\citenamefont {Altrock}, \citenamefont {Liu},\ and\ \citenamefont {Michor}}]{altrockMathematicsCancerIntegrating2015}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.~M.}\ \bibnamefont {Altrock}}, \bibinfo {author} {\bibfnamefont {L.~L.}\ \bibnamefont {Liu}},\ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Michor}},\ }\bibfield  {title} {\bibinfo {title} {The mathematics of cancer: Integrating quantitative models},\ }\href {https://doi.org/10.1038/nrc4029} {\bibfield  {journal} {\bibinfo  {journal} {Nature Reviews Cancer}\ }\textbf {\bibinfo {volume} {15}},\ \bibinfo {pages} {730} (\bibinfo {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Norton}\ \emph {et~al.}(2019)\citenamefont {Norton}, \citenamefont {Gong}, \citenamefont {Jamalian},\ and\ \citenamefont {Popel}}]{nortonMultiscaleAgentBasedHybrid2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.-A.}\ \bibnamefont {Norton}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Gong}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Jamalian}},\ and\ \bibinfo {author} {\bibfnamefont {A.~S.}\ \bibnamefont {Popel}},\ }\bibfield  {title} {\bibinfo {title} {Multiscale {{Agent-Based}} and {{Hybrid Modeling}} of the {{Tumor Immune Microenvironment}}},\ }\href {https://doi.org/10.3390/pr7010037} {\bibfield  {journal} {\bibinfo  {journal} {Processes}\ }\textbf {\bibinfo {volume} {7}},\ \bibinfo {pages} {37} (\bibinfo {year} {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ghaffarizadeh}\ \emph {et~al.}(2018)\citenamefont {Ghaffarizadeh}, \citenamefont {Heiland}, \citenamefont {Friedman}, \citenamefont {Mumenthaler},\ and\ \citenamefont {Macklin}}]{ghaffarizadehPhysiCellOpenSource2018}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Ghaffarizadeh}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Heiland}}, \bibinfo {author} {\bibfnamefont {S.~H.}\ \bibnamefont {Friedman}}, \bibinfo {author} {\bibfnamefont {S.~M.}\ \bibnamefont {Mumenthaler}},\ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Macklin}},\ }\bibfield  {title} {\bibinfo {title} {{{PhysiCell}}: {{An}} open source physics-based cell simulator for 3-{{D}} multicellular systems},\ }\href {https://doi.org/10.1371/journal.pcbi.1005991} {\bibfield  {journal} {\bibinfo  {journal} {PLOS Computational Biology}\ }\textbf {\bibinfo {volume} {14}},\ \bibinfo {pages} {e1005991} (\bibinfo {year} {2018})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ghaffarizadeh}\ \emph {et~al.}(2016)\citenamefont {Ghaffarizadeh}, \citenamefont {Friedman},\ and\ \citenamefont {Macklin}}]{ghaffarizadehBioFVMEfficientParallelized2016}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Ghaffarizadeh}}, \bibinfo {author} {\bibfnamefont {S.~H.}\ \bibnamefont {Friedman}},\ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Macklin}},\ }\bibfield  {title} {\bibinfo {title} {{{BioFVM}}: An efficient, parallelized diffusive transport solver for 3-{{D}} biological simulations},\ }\href {https://doi.org/10.1093/bioinformatics/btv730} {\bibfield  {journal} {\bibinfo  {journal} {Bioinformatics}\ }\textbf {\bibinfo {volume} {32}},\ \bibinfo {pages} {1256} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Metzcar}\ \emph {et~al.}(2024)\citenamefont {Metzcar}, \citenamefont {Duggan}, \citenamefont {Fischer}, \citenamefont {Murphy}, \citenamefont {Heiland},\ and\ \citenamefont {Macklin}}]{metzcarSimpleFrameworkAgentbased2024}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Metzcar}}, \bibinfo {author} {\bibfnamefont {B.~S.}\ \bibnamefont {Duggan}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Fischer}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Murphy}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Heiland}},\ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Macklin}},\ }\href {https://doi.org/10.1101/2022.11.21.514608} {\bibinfo {title} {A simple framework for agent-based modeling with extracellular matrix}} (\bibinfo {year} {2024})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bergman}\ \emph {et~al.}(2022)\citenamefont {Bergman}, \citenamefont {Marazzi}, \citenamefont {Chowkwale}, \citenamefont {M}, \citenamefont {Bidanta}, \citenamefont {Mapder},\ and\ \citenamefont {Li}}]{bergmanPhysiPKPDPharmacokineticsPharmacodynamics2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Bergman}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Marazzi}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Chowkwale}}, \bibinfo {author} {\bibfnamefont {D.~M.}\ \bibnamefont {M}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Bidanta}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Mapder}},\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Li}},\ }\bibfield  {title} {\bibinfo {title} {{{PhysiPKPD}}: {{A}} pharmacokinetics and pharmacodynamics module for {{PhysiCell}}},\ }\href {https://doi.org/10.46471/gigabyte.72} {\bibfield  {journal} {\bibinfo  {journal} {Gigabyte}\ }\textbf {\bibinfo {volume} {2022}},\ \bibinfo {pages} {1} (\bibinfo {year} {2022})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{Ponce-de-Leon}}\ \emph {et~al.}(2023)\citenamefont {{Ponce-de-Leon}}, \citenamefont {Montagud}, \citenamefont {No{\"e}l}, \citenamefont {Meert}, \citenamefont {Pradas}, \citenamefont {Barillot}, \citenamefont {Calzone},\ and\ \citenamefont {Valencia}}]{ponce-de-leonPhysiBoSSSustainableIntegration2023a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {{Ponce-de-Leon}}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Montagud}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {No{\"e}l}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Meert}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Pradas}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Barillot}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Calzone}},\ and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Valencia}},\ }\bibfield  {title} {\bibinfo {title} {{{PhysiBoSS}} 2.0: A sustainable integration of stochastic {{Boolean}} and agent-based modelling frameworks},\ }\href {https://doi.org/10.1038/s41540-023-00314-4} {\bibfield  {journal} {\bibinfo  {journal} {npj Systems Biology and Applications}\ }\textbf {\bibinfo {volume} {9}},\ \bibinfo {pages} {1} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Stoll}\ \emph {et~al.}(2017)\citenamefont {Stoll}, \citenamefont {Caron}, \citenamefont {Viara}, \citenamefont {Dugourd}, \citenamefont {Zinovyev}, \citenamefont {Naldi}, \citenamefont {Kroemer}, \citenamefont {Barillot},\ and\ \citenamefont {Calzone}}]{stollMaBoSSEnvironmentStochastic2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Stoll}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Caron}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Viara}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Dugourd}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Zinovyev}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Naldi}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Kroemer}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Barillot}},\ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Calzone}},\ }\bibfield  {title} {\bibinfo {title} {{{MaBoSS}} 2.0: An environment for stochastic {{Boolean}} modeling},\ }\href {https://doi.org/10.1093/bioinformatics/btx123} {\bibfield  {journal} {\bibinfo  {journal} {Bioinformatics}\ }\textbf {\bibinfo {volume} {33}},\ \bibinfo {pages} {2226} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Letort}\ \emph {et~al.}(2019)\citenamefont {Letort}, \citenamefont {Montagud}, \citenamefont {Stoll}, \citenamefont {Heiland}, \citenamefont {Barillot}, \citenamefont {Macklin}, \citenamefont {Zinovyev},\ and\ \citenamefont {Calzone}}]{letortPhysiBoSSMultiscaleAgentbased2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Letort}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Montagud}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Stoll}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Heiland}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Barillot}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Macklin}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Zinovyev}},\ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Calzone}},\ }\bibfield  {title} {\bibinfo {title} {{{PhysiBoSS}}: A multi-scale agent-based modelling framework integrating physical dimension and cell signalling},\ }\href {https://doi.org/10.1093/bioinformatics/bty766} {\bibfield  {journal} {\bibinfo  {journal} {Bioinformatics}\ }\textbf {\bibinfo {volume} {35}},\ \bibinfo {pages} {1188} (\bibinfo {year} {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ruscone}\ \emph {et~al.}(2024)\citenamefont {Ruscone}, \citenamefont {Checcoli}, \citenamefont {Heiland}, \citenamefont {Barillot}, \citenamefont {Macklin}, \citenamefont {Calzone},\ and\ \citenamefont {No{\"e}l}}]{rusconeBuildingMultiscaleModels2024}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Ruscone}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Checcoli}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Heiland}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Barillot}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Macklin}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Calzone}},\ and\ \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {No{\"e}l}},\ }\bibfield  {title} {\bibinfo {title} {Building multiscale models with {{PhysiBoSS}}, an agent-based modeling tool},\ }\href {https://doi.org/10.1093/bib/bbae509} {\bibfield  {journal} {\bibinfo  {journal} {Briefings in Bioinformatics}\ }\textbf {\bibinfo {volume} {25}},\ \bibinfo {pages} {bbae509} (\bibinfo {year} {2024})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Akasiadis}\ \emph {et~al.}(2022)\citenamefont {Akasiadis}, \citenamefont {{Ponce-de-Leon}}, \citenamefont {Montagud}, \citenamefont {Michelioudakis}, \citenamefont {Atsidakou}, \citenamefont {Alevizos}, \citenamefont {Artikis}, \citenamefont {Valencia},\ and\ \citenamefont {Paliouras}}]{akasiadisParallelModelExploration2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Akasiadis}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {{Ponce-de-Leon}}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Montagud}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Michelioudakis}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Atsidakou}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Alevizos}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Artikis}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Valencia}},\ and\ \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Paliouras}},\ }\bibfield  {title} {\bibinfo {title} {Parallel {{Model Exploration}} for {{Tumor Treatment Simulations}}},\ }\href {https://doi.org/10.1111/coin.12515} {\bibfield  {journal} {\bibinfo  {journal} {Computational Intelligence}\ }\textbf {\bibinfo {volume} {38}},\ \bibinfo {pages} {1379} (\bibinfo {year} {2022})},\ \Eprint {https://arxiv.org/abs/2103.14132} {arXiv:2103.14132 [cs, q-bio]} \BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Zeyen}\ and\ \citenamefont {Pang}(2022)}]{zeyenTargetControlBoolean2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Zeyen}}\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Pang}},\ }\bibfield  {title} {\bibinfo {title} {Target {{Control}} of {{Boolean Networks}} with {{Permanent Edgetic Perturbations}}},\ }in\ \href {https://doi.org/10.1109/CDC51059.2022.9992790} {\emph {\bibinfo {booktitle} {2022 {{IEEE}} 61st {{Conference}} on {{Decision}} and {{Control}} ({{CDC}})}}}\ (\bibinfo {year} {2022})\ pp.\ \bibinfo {pages} {4236--4243}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Su}\ and\ \citenamefont {Pang}(2020)}]{suDynamicsbasedApproachTarget2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Su}}\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Pang}},\ }\bibfield  {title} {\bibinfo {title} {A {{Dynamics-based Approach}} for the {{Target Control}} of {{Boolean Networks}}},\ }in\ \href {https://doi.org/10.1145/3388440.3412464} {\emph {\bibinfo {booktitle} {Proceedings of the 11th {{ACM International Conference}} on {{Bioinformatics}}, {{Computational Biology}} and {{Health Informatics}}}}},\ \bibinfo {series and number} {{{BCB}} '20}\ (\bibinfo  {publisher} {Association for Computing Machinery},\ \bibinfo {address} {New York, NY, USA},\ \bibinfo {year} {2020})\ pp.\ \bibinfo {pages} {1--8}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Newby}\ \emph {et~al.}(2023)\citenamefont {Newby}, \citenamefont {Za{\~n}udo},\ and\ \citenamefont {Albert}}]{newbyStructurebasedApproachIdentify2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Newby}}, \bibinfo {author} {\bibfnamefont {J.~G.~T.}\ \bibnamefont {Za{\~n}udo}},\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Albert}},\ }\bibfield  {title} {\bibinfo {title} {Structure-based approach to identify driver nodes in ensembles of biologically inspired {{Boolean}} networks},\ }\href {https://doi.org/10.1103/PhysRevResearch.5.033009} {\bibfield  {journal} {\bibinfo  {journal} {Physical Review Research}\ }\textbf {\bibinfo {volume} {5}},\ \bibinfo {pages} {033009} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Parmer}\ and\ \citenamefont {Rocha}(2023)}]{parmerDynamicalModularityAutomata2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Parmer}}\ and\ \bibinfo {author} {\bibfnamefont {L.~M.}\ \bibnamefont {Rocha}},\ }\href {https://doi.org/10.48550/arXiv.2303.16361} {\bibinfo {title} {Dynamical {{Modularity}} in {{Automata Models}} of {{Biochemical Networks}}}} (\bibinfo {year} {2023}),\ \Eprint {https://arxiv.org/abs/2303.16361} {arXiv:2303.16361 [cs, q-bio]} \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zhang}\ \emph {et~al.}(2008)\citenamefont {Zhang}, \citenamefont {Shah}, \citenamefont {Yang}, \citenamefont {Nyland}, \citenamefont {Liu}, \citenamefont {Yun}, \citenamefont {Albert},\ and\ \citenamefont {Loughran}}]{zhangNetworkModelSurvival2008}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Zhang}}, \bibinfo {author} {\bibfnamefont {M.~V.}\ \bibnamefont {Shah}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Yang}}, \bibinfo {author} {\bibfnamefont {S.~B.}\ \bibnamefont {Nyland}}, \bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Liu}}, \bibinfo {author} {\bibfnamefont {J.~K.}\ \bibnamefont {Yun}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Albert}},\ and\ \bibinfo {author} {\bibfnamefont {T.~P.}\ \bibnamefont {Loughran}},\ }\bibfield  {title} {\bibinfo {title} {Network model of survival signaling in large granular lymphocyte leukemia},\ }\href {https://doi.org/10.1073/pnas.0806447105} {\bibfield  {journal} {\bibinfo  {journal} {Proceedings of the National Academy of Sciences}\ }\textbf {\bibinfo {volume} {105}},\ \bibinfo {pages} {16308} (\bibinfo {year} {2008})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rozum}\ \emph {et~al.}(2021)\citenamefont {Rozum}, \citenamefont {G{\'o}mez Tejeda~Za{\~n}udo}, \citenamefont {Gan}, \citenamefont {Deritei},\ and\ \citenamefont {Albert}}]{rozumParityTimeReversal2021a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~C.}\ \bibnamefont {Rozum}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {G{\'o}mez Tejeda~Za{\~n}udo}}, \bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Gan}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Deritei}},\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Albert}},\ }\bibfield  {title} {\bibinfo {title} {Parity and time reversal elucidate both decision-making in empirical models and attractor scaling in critical {{Boolean}} networks},\ }\href {https://doi.org/10.1126/sciadv.abf8124} {\bibfield  {journal} {\bibinfo  {journal} {Science Advances}\ }\textbf {\bibinfo {volume} {7}},\ \bibinfo {pages} {eabf8124} (\bibinfo {year} {2021})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rozum}\ \emph {et~al.}(2022)\citenamefont {Rozum}, \citenamefont {Deritei}, \citenamefont {Park}, \citenamefont {G{\'o}mez Tejeda~Za{\~n}udo},\ and\ \citenamefont {Albert}}]{rozumPystablemotifsPythonLibrary2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~C.}\ \bibnamefont {Rozum}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Deritei}}, \bibinfo {author} {\bibfnamefont {K.~H.}\ \bibnamefont {Park}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {G{\'o}mez Tejeda~Za{\~n}udo}},\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Albert}},\ }\bibfield  {title} {\bibinfo {title} {Pystablemotifs: {{Python}} library for attractor identification and control in {{Boolean}} networks},\ }\href {https://doi.org/10.1093/bioinformatics/btab825} {\bibfield  {journal} {\bibinfo  {journal} {Bioinformatics}\ }\textbf {\bibinfo {volume} {38}},\ \bibinfo {pages} {1465} (\bibinfo {year} {2022})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Parmer}\ \emph {et~al.}(2022)\citenamefont {Parmer}, \citenamefont {Rocha},\ and\ \citenamefont {Radicchi}}]{parmerInfluenceMaximizationBoolean2022}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Parmer}}, \bibinfo {author} {\bibfnamefont {L.~M.}\ \bibnamefont {Rocha}},\ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Radicchi}},\ }\bibfield  {title} {\bibinfo {title} {Influence maximization in {{Boolean}} networks {\textbar} {{Nature Communications}}},\ }\href {https://doi.org/10.1038/s41467-022-31066-0} {\bibfield  {journal} {\bibinfo  {journal} {Nature Communications}\ }\textbf {\bibinfo {volume} {13}},\ \bibinfo {pages} {3457} (\bibinfo {year} {2022})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Campbell}\ and\ \citenamefont {Albert}(2019)}]{campbellEdgeticPerturbationsEliminate2019}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Campbell}}\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Albert}},\ }\bibfield  {title} {\bibinfo {title} {Edgetic perturbations to eliminate fixed-point attractors in {{Boolean}} regulatory networks},\ }\href {https://doi.org/10.1063/1.5083060} {\bibfield  {journal} {\bibinfo  {journal} {Chaos: An Interdisciplinary Journal of Nonlinear Science}\ }\textbf {\bibinfo {volume} {29}},\ \bibinfo {pages} {023130} (\bibinfo {year} {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Za{\~n}udo}\ and\ \citenamefont {Albert}(2015)}]{zanudoCellFateReprogramming2015}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~G.~T.}\ \bibnamefont {Za{\~n}udo}}\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Albert}},\ }\bibfield  {title} {\bibinfo {title} {Cell {{Fate Reprogramming}} by {{Control}} of {{Intracellular Network Dynamics}}},\ }\href {https://doi.org/10.1371/journal.pcbi.1004193} {\bibfield  {journal} {\bibinfo  {journal} {PLOS Computational Biology}\ }\textbf {\bibinfo {volume} {11}},\ \bibinfo {pages} {e1004193} (\bibinfo {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Park}\ \emph {et~al.}(2023)\citenamefont {Park}, \citenamefont {Costa}, \citenamefont {Rocha}, \citenamefont {Albert},\ and\ \citenamefont {Rozum}}]{parkModelsCellProcesses2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.~H.}\ \bibnamefont {Park}}, \bibinfo {author} {\bibfnamefont {F.~X.}\ \bibnamefont {Costa}}, \bibinfo {author} {\bibfnamefont {L.~M.}\ \bibnamefont {Rocha}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Albert}},\ and\ \bibinfo {author} {\bibfnamefont {J.~C.}\ \bibnamefont {Rozum}},\ }\bibfield  {title} {\bibinfo {title} {Models of {{Cell Processes}} are {{Far}} from the {{Edge}} of {{Chaos}}},\ }\href {https://doi.org/10.1103/PRXLife.1.023009} {\bibfield  {journal} {\bibinfo  {journal} {PRX Life}\ }\textbf {\bibinfo {volume} {1}},\ \bibinfo {pages} {023009} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Helikar}\ \emph {et~al.}(2012)\citenamefont {Helikar}, \citenamefont {Kowal}, \citenamefont {McClenathan}, \citenamefont {Bruckner}, \citenamefont {Rowley}, \citenamefont {Madrahimov}, \citenamefont {Wicks}, \citenamefont {Shrestha}, \citenamefont {Limbu},\ and\ \citenamefont {Rogers}}]{helikarCellCollectiveOpen2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Helikar}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Kowal}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {McClenathan}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Bruckner}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Rowley}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Madrahimov}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Wicks}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Shrestha}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Limbu}},\ and\ \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Rogers}},\ }\bibfield  {title} {\bibinfo {title} {The {{Cell Collective}}: {{Toward}} an open and collaborative approach to systems biology},\ }\href {https://doi.org/10.1186/1752-0509-6-96} {\bibfield  {journal} {\bibinfo  {journal} {BMC Systems Biology}\ }\textbf {\bibinfo {volume} {6}},\ \bibinfo {pages} {96} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Johnson}\ \emph {et~al.}(2023)\citenamefont {Johnson}, \citenamefont {{Stein-O'Brien}}, \citenamefont {Booth}, \citenamefont {Heiland}, \citenamefont {Kurtoglu}, \citenamefont {Bergman}, \citenamefont {Bucher}, \citenamefont {Deshpande}, \citenamefont {Forjaz}, \citenamefont {Getz}, \citenamefont {Godet}, \citenamefont {Lyman}, \citenamefont {Metzcar}, \citenamefont {Mitchell}, \citenamefont {Raddatz}, \citenamefont {Rocha}, \citenamefont {Solorzano}, \citenamefont {Sundus}, \citenamefont {Wang}, \citenamefont {Gilkes}, \citenamefont {Kagohara}, \citenamefont {Kiemen}, \citenamefont {Thompson}, \citenamefont {Wirtz}, \citenamefont {Wu}, \citenamefont {Zaidi}, \citenamefont {Zheng}, \citenamefont {Zimmerman}, \citenamefont {Jaffee}, \citenamefont {Chang}, \citenamefont {Coussens}, \citenamefont {Gray}, \citenamefont {Heiser}, \citenamefont {Fertig},\ and\ \citenamefont {Macklin}}]{johnsonDigitizeYourBiology2023a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~A.~I.}\ \bibnamefont {Johnson}}, \bibinfo {author} {\bibfnamefont {G.~L.}\ \bibnamefont {{Stein-O'Brien}}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Booth}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Heiland}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Kurtoglu}}, \bibinfo {author} {\bibfnamefont {D.~R.}\ \bibnamefont {Bergman}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Bucher}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Deshpande}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Forjaz}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Getz}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Godet}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Lyman}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Metzcar}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Mitchell}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Raddatz}}, \bibinfo {author} {\bibfnamefont
  {H.}~\bibnamefont {Rocha}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Solorzano}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Sundus}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Wang}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Gilkes}}, \bibinfo {author} {\bibfnamefont {L.~T.}\ \bibnamefont {Kagohara}}, \bibinfo {author} {\bibfnamefont {A.~L.}\ \bibnamefont {Kiemen}}, \bibinfo {author} {\bibfnamefont {E.~D.}\ \bibnamefont {Thompson}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Wirtz}}, \bibinfo {author} {\bibfnamefont {P.-H.}\ \bibnamefont {Wu}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Zaidi}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Zheng}}, \bibinfo {author} {\bibfnamefont {J.~W.}\ \bibnamefont {Zimmerman}}, \bibinfo {author} {\bibfnamefont {E.~M.}\ \bibnamefont {Jaffee}}, \bibinfo {author} {\bibfnamefont {Y.~H.}\ \bibnamefont {Chang}}, \bibinfo {author} {\bibfnamefont {L.~M.}\ \bibnamefont {Coussens}}, \bibinfo {author}
  {\bibfnamefont {J.~W.}\ \bibnamefont {Gray}}, \bibinfo {author} {\bibfnamefont {L.~M.}\ \bibnamefont {Heiser}}, \bibinfo {author} {\bibfnamefont {E.~J.}\ \bibnamefont {Fertig}},\ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Macklin}},\ }\href {https://doi.org/10.1101/2023.09.17.557982} {\bibinfo {title} {Digitize your {{Biology}}! {{Modeling}} multicellular systems through interpretable cell behavior}} (\bibinfo {year} {2023})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Correia}\ \emph {et~al.}(2018)\citenamefont {Correia}, \citenamefont {Gates}, \citenamefont {Wang},\ and\ \citenamefont {Rocha}}]{correiaCANAPythonPackage2018}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.~B.}\ \bibnamefont {Correia}}, \bibinfo {author} {\bibfnamefont {A.~J.}\ \bibnamefont {Gates}}, \bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Wang}},\ and\ \bibinfo {author} {\bibfnamefont {L.~M.}\ \bibnamefont {Rocha}},\ }\bibfield  {title} {\bibinfo {title} {{{CANA}}: {{A Python Package}} for {{Quantifying Control}} and {{Canalization}} in {{Boolean Networks}}},\ }\bibfield  {journal} {\bibinfo  {journal} {Frontiers in Physiology}\ }\textbf {\bibinfo {volume} {9}},\ \href {https://doi.org/10.3389/fphys.2018.01046} {10.3389/fphys.2018.01046} (\bibinfo {year} {2018})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Albert}\ \emph {et~al.}(2008)\citenamefont {Albert}, \citenamefont {Thakar}, \citenamefont {Li}, \citenamefont {Zhang},\ and\ \citenamefont {Albert}}]{albertBooleanNetworkSimulations2008}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Albert}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Thakar}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Li}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Zhang}},\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Albert}},\ }\bibfield  {title} {\bibinfo {title} {Boolean network simulations for life scientists},\ }\href {https://doi.org/10.1186/1751-0473-3-16} {\bibfield  {journal} {\bibinfo  {journal} {Source Code for Biology and Medicine}\ }\textbf {\bibinfo {volume} {3}},\ \bibinfo {pages} {16} (\bibinfo {year} {2008})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Paulev{\'e}}\ \emph {et~al.}(2020)\citenamefont {Paulev{\'e}}, \citenamefont {Kol{\v c}{\'a}k}, \citenamefont {Chatain},\ and\ \citenamefont {Haar}}]{pauleveReconcilingQualitativeAbstract2020a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Paulev{\'e}}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Kol{\v c}{\'a}k}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Chatain}},\ and\ \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Haar}},\ }\bibfield  {title} {\bibinfo {title} {Reconciling qualitative, abstract, and scalable modeling of biological networks},\ }\href {https://doi.org/10.1038/s41467-020-18112-5} {\bibfield  {journal} {\bibinfo  {journal} {Nature Communications}\ }\textbf {\bibinfo {volume} {11}},\ \bibinfo {pages} {4256} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{Leonard-Duke}}\ \emph {et~al.}(2020)\citenamefont {{Leonard-Duke}}, \citenamefont {Evans}, \citenamefont {Hannan}, \citenamefont {Barker}, \citenamefont {Bates}, \citenamefont {Bonham}, \citenamefont {Moore}, \citenamefont {Kirschner},\ and\ \citenamefont {Peirce}}]{leonard-dukeMultiscaleModelsLung2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {{Leonard-Duke}}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Evans}}, \bibinfo {author} {\bibfnamefont {R.~T.}\ \bibnamefont {Hannan}}, \bibinfo {author} {\bibfnamefont {T.~H.}\ \bibnamefont {Barker}}, \bibinfo {author} {\bibfnamefont {J.~H.}\ \bibnamefont {Bates}}, \bibinfo {author} {\bibfnamefont {C.~A.}\ \bibnamefont {Bonham}}, \bibinfo {author} {\bibfnamefont {B.~B.}\ \bibnamefont {Moore}}, \bibinfo {author} {\bibfnamefont {D.~E.}\ \bibnamefont {Kirschner}},\ and\ \bibinfo {author} {\bibfnamefont {S.~M.}\ \bibnamefont {Peirce}},\ }\bibfield  {title} {\bibinfo {title} {Multi-scale models of lung fibrosis},\ }\href {https://doi.org/10.1016/j.matbio.2020.04.003} {\bibfield  {journal} {\bibinfo  {journal} {Matrix Biology}\ }\textbf {\bibinfo {volume} {91--92}},\ \bibinfo {pages} {35} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Craig}\ \emph {et~al.}(2023)\citenamefont {Craig}, \citenamefont {Gevertz}, \citenamefont {Kareva},\ and\ \citenamefont {Wilkie}}]{craigPracticalGuideGeneration2023}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Craig}}, \bibinfo {author} {\bibfnamefont {J.~L.}\ \bibnamefont {Gevertz}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Kareva}},\ and\ \bibinfo {author} {\bibfnamefont {K.~P.}\ \bibnamefont {Wilkie}},\ }\bibfield  {title} {\bibinfo {title} {A practical guide for the generation of model-based virtual clinical trials},\ }\bibfield  {journal} {\bibinfo  {journal} {Frontiers in Systems Biology}\ }\textbf {\bibinfo {volume} {3}},\ \href {https://doi.org/10.3389/fsysb.2023.1174647} {10.3389/fsysb.2023.1174647} (\bibinfo {year} {2023})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Metzcar}\ \emph {et~al.}(2025)\citenamefont {Metzcar}, \citenamefont {Guenter}, \citenamefont {Wang}, \citenamefont {Baker},\ and\ \citenamefont {Lines}}]{metzcarImprovingNeuroendocrineTumor2025}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~P.}\ \bibnamefont {Metzcar}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Guenter}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Wang}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Baker}},\ and\ \bibinfo {author} {\bibfnamefont {K.~E.}\ \bibnamefont {Lines}},\ }\bibfield  {title} {\bibinfo {title} {Improving neuroendocrine tumor treatments with mathematical modeling: Lessons from other endocrine cancers}\ }\href {https://doi.org/10.1530/EO-24-0025} {10.1530/EO-24-0025} (\bibinfo {year} {2025})\BibitemShut {NoStop}%
\end{thebibliography}%

